DiffusionLight-Turbo: Accelerated Light Probes for Free via Single-Pass Chrome Ball Inpainting

We introduce a simple yet effective technique for estimating lighting from a single low-dynamic-range (LDR) image by reframing the task as a chrome ball inpainting problem. This approach leverages a pre-trained diffusion model, Stable Diffusion XL, to overcome the generalization failures of existing methods that rely on limited HDR panorama datasets. While conceptually simple, the task remains challenging because diffusion models often insert incorrect or inconsistent content and cannot readily generate chrome balls in HDR format. Our analysis reveals that the inpainting process is highly sensitive to the initial noise in the diffusion process, occasionally resulting in unrealistic outputs. To address this, we first introduce DiffusionLight, which uses iterative inpainting to compute a median chrome ball from multiple outputs to serve as a stable, low-frequency lighting prior that guides the generation of a high-quality final result. To generate high-dynamic-range (HDR) light probes, an Exposure LoRA is fine-tuned to create LDR images at multiple exposure values, which are then merged. While effective, DiffusionLight is time-intensive, requiring approximately 30 minutes per estimation. To reduce this overhead, we introduce DiffusionLight-Turbo, which reduces the runtime to about 30 seconds with minimal quality loss. This 60x speedup is achieved by training a Turbo LoRA to directly predict the averaged chrome balls from the iterative process. Inference is further streamlined into a single denoising pass using a LoRA swapping technique. Experimental results that show our method produces convincing light estimates across diverse settings and demonstrates superior generalization to in-the-wild scenarios. Our code is available at https://diffusionlight.github.io/turbo

==> figs/additional_object_insertion_halfpage.tex <==
% ==============================
% Additional Result for object insertion
% ===============================

\tabulinesep=0.5pt
\begin{figure*}[!t]
    \centering

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
    }

        \multicolumn{1}{c}{\shortstack{ Input object}}
        &
        \multicolumn{1}{c}{\shortstack{Input object}} \\
        \noindent\parbox[c]{0.5\textwidth}{\centering\includegraphics[height=0.2\textwidth]{storage/appendix_object_insertion/input_bag.pdf}} &
        \noindent\parbox[c]{0.5\textwidth}{\centering\includegraphics[height=0.2\textwidth]{storage/appendix_object_insertion/input_shoe.pdf}}
    \end{tabu}

    \begin{tabu} to \textwidth {
        @{}
        % 1st example
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
    }

        \multicolumn{1}{c}{\shortstack{ Before relighting}}
        &
        \multicolumn{1}{c}{\shortstack{ After relighting}}
        &
        \multicolumn{1}{c}{\shortstack{ Before relighting}}
        &
        \multicolumn{1}{c}{\shortstack{ After relighting}}
        \\ 
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_bag_no_light.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_bag.pdf}}&
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_shoe_no_light.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/bedzoom_shoe.pdf}}
        % bag
        \\
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_bag_nolight.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_bag.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_shoe_nolight.pdf}} &
        \noindent\parbox[c]{0.23\textwidth}{\includegraphics[height=0.23\textwidth]{storage/appendix_object_insertion_perspective/cambodia2tilt_shoe.pdf}}
    \end{tabu}
    \caption{
    We synthetically render each 3D object into input images using our estimated lighting.
    %results for virtual object insertion.
    }
    \label{fig:additional_object_insertion}
\end{figure*}

==> figs/teaser_rev2.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\vspace{-3em}
\begin{center}
    \centering
    \captionsetup{type=figure}
    \includegraphics[width=1.0\textwidth]{figs/teaser_rev2.pdf}
    \captionof{figure}{\textbf{DiffusionLight-Turbo} leverages a pre-trained diffusion model (Stable Diffusion XL) for light estimation by rendering an HDR chrome ball. In each scene, we show our normally exposed chrome ball on top and our underexposed version, which reveals bright light sources, on the bottom. 
    } \label{fig:teaser}
\end{center}%
}]

==> tables/ldr_stylelight.tex <==
\begin{table}[!h]
\centering
\small

\caption{
    Scores on LDR environment maps (Section~\ref{sec:ldr-panoramas-eval}). 
}
\label{tab:ldr-stylelight}

\begin{tabular}{
    l@{\hspace{5pt}}
    l@{\hspace{5pt}}
    c@{\hspace{5pt}}
    c@{\hspace{5pt}}
    c
}
\toprule
\textbf{Dataset} & \textbf{Method} & \textbf{RMSE} $\downarrow$ & \textbf{si-RMSE} $\downarrow$ & \begin{tabular}[c]{@{}c@{}}\textbf{Angular}\\ \textbf{Error}\end{tabular} $\downarrow$\\
\midrule

Laval Indoor \cite{garder2017lavelindoor} & StyleLight & 0.246 & \colorbox{tabfirst}{0.271} & 5.814\\
 & \textbf{Ours} & \colorbox{tabfirst}{0.187} & 0.303 & \colorbox{tabfirst}{4.412} \\
 \hline
 Poly Haven  \cite{polyhaven}& StyleLight & 0.241 & 0.324 & 6.291 \\
 & \textbf{Ours} & \colorbox{tabfirst}{0.179} & \colorbox{tabfirst}{0.275} & \colorbox{tabfirst}{4.567} \\

\bottomrule
\end{tabular}
\end{table}

==> tables/polyhaven_stylelight.tex <==
\begin{table}[t]
\centering
\caption{
Comparison with previous work on Mirror / Matte / Diffuse sphere rendering on PolyHaven Dataset
}
\label{tab:polyhaven-stylelight}

\begin{tabular}{llccc}
\toprule
    Sphere & Method &  Angular Error \downarrow & RMSE \downarrow & si-RMSE \downarrow \\
    \midrule
    \multirow{3}{*}{Diffuse}
    & Stylelight \cite{wang2022stylelight}  & 0.67 & 0.41 & 7.12 \\
    & Ours & 0.36 & 0.14 & 2.14 \\
    \midrule    
    \multirow{3}{*}{Matte}
    & Stylelight \cite{wang2022stylelight}  & 0.56  & 0.28 & 4.44 \\
    & Ours & 0.64 & 0.45 & 3.60 \\
    \midrule
    \multirow{3}{*}{Mirror}
    & Stylelight \cite{wang2022stylelight}  & 0.30 & 0.12 & 3.53\\
    & Ours & 0.86 & 0.67 & 4.31 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/render_stylelight_backup.tex <==
\begin{table*}[!h]
\centering
\small
% \caption{Comparison using the three-sphere evaluation protocol between StyleLight \cite{wang2022stylelight}, simple inpainting with SDXL \cite{podell2023sdxl} and depth-conditioned ControlNet \cite{zhang2023adding}  (``SDXL$^\dagger$'' in the table), and ablated versions of our method. The \colorbox{tabfirst}{best} and \colorbox{tabsecond}{second-best}are color coded.}
\caption{Scores on three-sphere evaluation protocol. The \colorbox{tabfirst}{best} and \colorbox{tabsecond}{second-best}are color-coded.}
\label{tab:indoor_stylelight}

\resizebox{1\textwidth}{!}{%
\setlength{\tabcolsep}{1pt}
\begin{tabular}{
    l@{\hspace{9pt}}
    l@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c
}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Scale-invariant RMSE} $\downarrow$} & \multicolumn{3}{c}{\textbf{Angular Error} $\downarrow$}  & \multicolumn{3}{c}{\textbf{Normalized RMSE} $\downarrow$}                                                            \\
 & & Diffuse           & Matte           & Mirror           & Diffuse           & Matte           & Mirror   & Diffuse           & Matte           & Mirror      \\ 
\midrule

Laval Indoor \cite{garder2017lavelindoor} & StyleLight {\footnotesize(reported by the paper)} & 0.11 & 0.29 & 0.55 & 2.41 & 2.96 & 4.30 & - & - & - \\

\hline

\multirow{5}{*}{Laval Indoor \cite{garder2017lavelindoor}}  & StyleLight {\footnotesize (reproduced using official code)} & 0.135 & 0.315 & 0.552 & 4.238 & 4.742 & 6.781 & 0.234 & 0.404 & 0.511 \\
& SDXL$^\dagger$ & 0.196 & 0.453 & 0.715 & 5.867 & 6.196 & 8.279 & 0.320 & 0.475 & 0.510 \\
& SDXL$^\dagger$ + iterative (ours) & 0.146 & 0.388 & 0.669 & 3.581 & 4.551 & 7.053 & 0.246 & 0.408 & 0.467 \\
& SDXL$^\dagger$ + LoRA (ours) & 0.147 & 0.380 & 0.651 & 3.470 & 3.864 & 6.146 & 0.255 & 0.397 & 0.451 \\
& SDXL$^\dagger$ + iterative + LoRA (ours) & 0.140 & 0.325 & 0.597 & 2.139 & 3.421 & 5.936 & 0.201 & 0.361 & 0.431 \\

\hline

\multirow{5}{*}{Poly Haven \cite{polyhaven}} & StyleLight {\footnotesize (reproduced using official code)} & 0.166 & 0.441 & 0.639 & 3.533 & 4.438 & 7.122 & 0.225 & 0.415 & 0.488 \\
& SDXL$^\dagger$ & 0.218 & 0.585 & 0.804 & 2.983 & 4.252 & 5.738 & 0.296 & 0.504 & 0.543 \\
& SDXL$^\dagger$ + iterative (ours) & 0.161 & 0.500 & 0.735 & 2.574 & 4.183 & 5.306 & 0.221 & 0.443 & 0.495 \\
& SDXL$^\dagger$ + LoRA (ours) & 0.165 & 0.499 & 0.718 & 2.352 & 3.560 & 4.433 & 0.235 & 0.430 & 0.47 \\
& SDXL$^\dagger$ + iterative + LoRA (ours) & 0.140 & 0.446 & 0.664 & 2.139 & 3.595 & 4.286 & 0.201 & 0.388 & 0.428 \\

%%%%%%%%%%%%%%
% INDOOR
% StyleLight (Paper) \cite{wang2022stylelight} & 0.11 & 0.29 & 0.55 & 2.41 & 2.96 & 4.30 & - & - & - \\
%%%%%%%%%%%%%%
\bottomrule
\addlinespace[0.2em]
\multicolumn{11}{l}{\textit{SDXL$^\dagger$ denotes simple inpainting with SDXL \cite{podell2023sdxl} and depth-conditioned ControlNet \cite{zhang2023adding}}.} \\
\end{tabular}}
\end{table*}

==> tables/render_stylelight_ver2.tex <==
\begin{table*}[!h]
\centering
\small
% \caption{Comparison using the three-sphere evaluation protocol between StyleLight \cite{wang2022stylelight}, simple inpainting with SDXL \cite{podell2023sdxl} and depth-conditioned ControlNet \cite{zhang2023adding}  (``SDXL$^\dagger$'' in the table), and ablated versions of our method. The \colorbox{tabfirst}{best} and \colorbox{tabsecond}{second-best}are color coded.}
\caption{Scores on three-sphere evaluation protocol. The \colorbox{tabfirst}{best} and \colorbox{tabsecond}{second-best}are color-coded.}
\label{tab:indoor_stylelight}

\resizebox{1\textwidth}{!}{%
\setlength{\tabcolsep}{1pt}
\begin{tabular}{
    l@{\hspace{9pt}}
    l@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c@{\hspace{9pt}}
    c
}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Scale-invariant RMSE} $\downarrow$} & \multicolumn{3}{c}{\textbf{Angular Error} $\downarrow$}  & \multicolumn{3}{c}{\textbf{Normalized RMSE} $\downarrow$}                                                            \\
 & & Diffuse           & Matte           & Mirror           & Diffuse           & Matte           & Mirror   & Diffuse           & Matte           & Mirror      \\ 
\midrule

Laval Indoor \cite{garder2017lavelindoor} & StyleLight {\footnotesize(reported by the paper)} & 0.11 & 0.29 & 0.55 & 2.41 & 2.96 & 4.30 & - & - & - \\

\hline

\multirow{5}{*}{Laval Indoor \cite{garder2017lavelindoor}}  & StyleLight {\footnotesize (reproduced using official code)} & 0.13 & 0.31 & 0.55 & 4.24 & 4.74 & 6.78 & \colorbox{tabsecond}{0.23} & \colorbox{tabsecond}{0.40} & 0.51 \\
& SDXL$^\dagger$ & 0.20 & 0.45 & 0.72 & 5.87 & 6.20 & 8.28 & 0.32 & 0.47 & 0.51 \\
& SDXL$^\dagger$ + iterative (ours) & 0.15 & 0.39 & 0.67 & 3.58 & 4.55 & 7.05 & 0.25 & 0.41 & 0.47 \\
& SDXL$^\dagger$ + LoRA (ours) & 0.15 & 0.38 & 0.65 & \colorbox{tabsecond}{3.47} & \colorbox{tabsecond}{3.86} & \colorbox{tabsecond}{6.15} & 0.25 & \colorbox{tabsecond}{0.40} & \colorbox{tabsecond}{0.45} \\
& SDXL$^\dagger$ + iterative + LoRA (ours) & \colorbox{tabsecond}{0.14} & \colorbox{tabsecond}{0.33} & \colorbox{tabsecond}{0.60} & \colorbox{tabfirst}{2.14} & \colorbox{tabfirst}{3.42} & \colorbox{tabfirst}{5.94} & \colorbox{tabfirst}{0.20} & \colorbox{tabfirst}{0.36} & \colorbox{tabfirst}{0.43} \\

\hline

\multirow{5}{*}{Poly Haven \cite{polyhaven}} & StyleLight {\footnotesize (reproduced using official code)} & 0.17 & \colorbox{tabfirst}{0.44} & \colorbox{tabfirst}{0.64} & 3.53 & 4.44 & 7.12 & 0.23 & \colorbox{tabsecond}{0.41} & 0.49 \\
& SDXL$^\dagger$ & 0.22 & 0.59 & 0.80 & 2.98 & 4.25 & 5.74 & 0.30 & 0.50 & 0.54 \\
& SDXL$^\dagger$ + iterative (ours) & \colorbox{tabsecond}{0.16} & 0.50 & 0.73 & 2.57 & 4.18 & 5.31 & \colorbox{tabsecond}{0.22} & 0.44 & 0.50 \\
& SDXL$^\dagger$ + LoRA (ours) & \colorbox{tabsecond}{0.16} & 0.50 & 0.72 & \colorbox{tabsecond}{2.35} & \colorbox{tabfirst}{3.56} & \colorbox{tabsecond}{4.43} & 0.24 & 0.43 & \colorbox{tabsecond}{0.47} \\
& SDXL$^\dagger$ + iterative + LoRA (ours) & \colorbox{tabfirst}{0.14} & \colorbox{tabsecond}{0.45} & \colorbox{tabsecond}{0.66} & \colorbox{tabfirst}{2.14} & \colorbox{tabsecond}{3.60} & \colorbox{tabfirst}{4.29} & \colorbox{tabfirst}{0.20} & \colorbox{tabfirst}{0.39} & \colorbox{tabfirst}{0.43} \\

%%%%%%%%%%%%%%
% INDOOR
% StyleLight (Paper) \cite{wang2022stylelight} & 0.11 & 0.29 & 0.55 & 2.41 & 2.96 & 4.30 & - & - & - \\
%%%%%%%%%%%%%%
\bottomrule
\addlinespace[0.2em]
\multicolumn{11}{l}{\textit{SDXL$^\dagger$ denotes simple inpainting with SDXL \cite{podell2023sdxl} and depth-conditioned ControlNet \cite{zhang2023adding}}.} \\
\end{tabular}}
\end{table*}
